Probing Cosmic Inflation with the LiteBIRD Cosmic Microwave Background Polarization Survey

LiteBIRD, the Lite (Light) satellite for the study of B-mode polarization and Inflation from cosmic background Radiation Detection, is a space mission for primordial cosmology and fundamental physics. The Japan Aerospace Exploration Agency (JAXA) selected LiteBIRD in May 2019 as a strategic large-class (L-class) mission, with an expected launch in the late 2020s using JAXA's H3 rocket. LiteBIRD is planned to orbit the Sun-Earth Lagrangian point L2, where it will map the cosmic microwave background (CMB) polarization over the entire sky for three years, with three telescopes in 15 frequency bands between 34 and 448 GHz, to achieve an unprecedented total sensitivity of 2.2$\mu$K-arcmin, with a typical angular resolution of 0.5$^\circ$ at 100 GHz. The primary scientific objective of LiteBIRD is to search for the signal from cosmic inflation, either making a discovery or ruling out well-motivated inflationary models. The measurements of LiteBIRD will also provide us with insight into the quantum nature of gravity and other new physics beyond the standard models of particle physics and cosmology. We provide an overview of the LiteBIRD project, including scientific objectives, mission and system requirements, operation concept, spacecraft and payload module design, expected scientific outcomes, potential design extensions and synergies with other projects.

==> acronymes_table.tex <==
\begin{table}
\begin{tabular}{|l|l|}
\hline
acronyme & definition \\
\hline
	2ST	&	Two-stage Stirling cooler	\\
%	4K-GM	&	4-K Gifford-McMahon (Cryocoolers)	\\
%	4K-JT	&	4-K Joule-Thomson cooler	\\
%	A4K	&	Amumetal 4-K magnetic shield	\\
%	AC	&	Alternating current	\\
%	ACT	&	Atacama Cosmology Telescope (a ground-based experiment)	\\
%	ADC	&	Analog-to-digital converter	\\
	ADR	&	Adiabatic demagnetization refrigerator	\\
%	ADRC	&	ADR controller	\\
%	AES	&	Advanced Engineering Services Co., Ltd.	\\
%	AHWP	&	Achromatic half-wave plate	\\
%	AIT	&	Assembly, integration, and testing	\\
%	AIV	&	Assembly, integration, and verification	\\
%	AME	&	Anomalous microwave emission	\\
%	AN72	&	A particular type of Eccosorb microwave absorber (http://www.eccosorb.com)	\\
	AOCS	&	Attitude orbit-control system	\\
%	APS	&	Angular power spectrum	\\
%	AR	&	Anti-reflection	\\
%	ARC	&	Anti-reflection coating	\\
%	ASI	&	Alenia Space Italia (Italian Space Agency)	\\
%	ASTM E595-15	&	Standard test method for outgassing (www.astm.org)	\\
%	BBM	&	Breadboard model	\\
%	BICEP	&	Background Imaging of Cosmic Extragalactic Polarization (experiment)	\\
%	BOL	&	Beginning of life	\\
%	BW	&	Band width	\\
%	CAD	&	Computer-aided design	\\
%	CAS	&	Cold aperture stop	\\
%	CATR	&	Compact antenna test range	\\
%	CCDR	&	Closed-cycle diluition refrigerator	\\
%	CDF	&	Concurrent Design Facility at ESA	\\
%	CDR	&	Critical design review	\\
%	CEA	&	French Alternative Energies and Atomic Energy Commission	\\
%	CEA/SBT	&	Service team of low temperatures of CEA	\\
%	CFRP	&	Carbon-fiber reinforced plastic	\\
	CMB	&	Cosmic microwave background	\\
	CMB-S4	&	CMB Stage-4 experiment	\\
%	CML	&	Concept maturity level	\\
%	CNES	&	Centre National d'Etudes Spatiales (French Space Agency)	\\
%	CO	&	Carbon monoxide	\\
	COBE	&	Cosmic Background Explorer (NASA satellite mission)	\\
%	COMSOL	&	Finite-element analysis software (www.comsol.com)	\\
%	CR110	&	A particular type of molded Eccosorb microwave absorber (http://www.eccosorb.com)	\\
%	CRHWP	&	Continuously-rotating half-wave plate	\\
%	CSA	&	Canadian Space Agency	\\
%	CT	&	Cryogenic test	\\
%	CVCM	&	Collected volatile condensable materials	\\
%	CW	&	Continuous wave	\\
%	DC	&	Direct current	\\
%	DM	&	Demonstration model	\\
%	DPU	&	Data processing unit	\\
%	E2E	&	End-to-end	\\
%	EBEX	&	"E and B EXperiment", a balloon-borne CMB experiment	\\
%	EM	&	Engineering model	\\
%	EMC/EMI	&	Electromagnetic compatibility	\\
%	EMI	&	Electromagnetic interference	\\
%	EOL	&	End of life	\\
%	EQM	&	Engineering qualification model	\\
%	ER-HWP	&	Embedded reflective half-wave plate	\\
%	ESA	&	European Space Agency	\\
%	FEM	&	Finite-element method	\\
%	FG	&	Foreground	\\
FLRW & Friedmann-Lemaître-Robertson-Walker model \\
%	FM	&	Flight model	\\
%	FOV	&	Field of view	\\
%	FP	&	Focal plane	\\
%	FPGA	&	Field-programmable gate array	\\
%	FPU	&	Focal-plane unit	\\
%	FSL	&	Far sidelobe	\\
%	FTA	&	Fault tree analysis	\\
%	FTS	&	Fourier-transform spectroscopy	\\
	FWHM	&	Full width at half maximum	\\
%	GAL060	&	A specific Galactic mask	\\
%	GM	&	Gifford-McMahon cooler	\\
%	GM100	&	A CMB sky simulation package	\\
%	GRASP	&	General Reflector Antenna Software Package (www.ticra.com)	\\
%	GSE	&	Ground Support Equipment	\\
%	HCE	&	heater control electronis	\\
%	HF	&	High frequency	\\
%	HFSS	&	High-frequency electromagnetic field simulator (www.ansys.com)	\\
%	HFT	&	High Frequency Telescope	\\
%	HIMAC	&	Heavy Ion Medical Accelerator (in Chiba, Japan)	\\
%	HK	&	Housekeeping	\\
%	HR10, HR25	&	Specific Eccosorb products (http://www.eccosorb.com)	\\
%	HWP	&	Half-wave plate	\\
%	IAS	&	Institut d’Astrophysique Spatiale (in Orsay, France)	\\
%	IDR/UPM	&	Institute of Microgravity "Ignacio Da Riva" of the Technical University of Madrid	\\
%	IGB	&	Interim Governance Board (of LiteBIRD)	\\
%	ILC	&	Internal linear combination	\\
%	IMO	&	Instrument MOdel (this is the data representing the design and performance parameters of the instrument, including processed data such as calculated beam profiles, but not software that predicts performance)	\\
%	INFN	&	Istituto Nazionale di Fisica Nucleare (Italian National Institute for Nuclear Physics)	\\
%	IP	&	Instrumental polarization	\\
%	IR	&	Infrared	\\
%	IRAM	&	Institut de Radioastronomie Millimétrique (Grenoble, France)	\\
%	IRAP	&	L'Institut de Recherche en Astrophysique et Planétologie (CNRS + Toulouse's Paul Sabatier University)	\\
IRU & Inertia reference unit \\
%	ISR	&	International Science Review (at ISAS/JAXA for LiteBIRD)	\\
%	ISS	&	International Space Station	\\
%	ITF	&	Internal template fitting	\\
JAXA &  Japan  Aerospace  Exploration  Agency \\
%	JMAG	&	Software for electromagnetic design (www.jmag-international.com)	\\
%	JSG	&	Joint Study Group (in LiteBIRD collaboration)	\\
%	JTD	&	Joule-Thomson cooler driver	\\
%	KAGRA	&	Kamioka Gravitational Wave Detector	\\
L2 & Second Lagrangian point \\
%	LAL	&	Laboratoire de l’Accélérateur Linéaire	\\
%	LBNL	&	Lawrence Berkeley National Laboratory ("Berkeley Lab")	\\
%	LC	&	Inductor capacitor	\\
%	LED	&	Light-emitting diode	\\
	LF	&	Low frequency	\\
	LFT	&	Low-Frequency Telescope	\\
	LiteBIRD	&	Lite (Light) satellite for the study of B-mode polarization and Inflation from cosmic background Radiation Detection	\\
%	LSPE/SWIPE	&	Large Scale Polarization Explorer - Short Wavelength Instrument for the Polarization Explorer	\\
%	LZH	&	Laser Zentrum Hannover (national lab in Germany)	\\
%	MDPU	&	Mission Data Processing Unit (synonyms: PLM-DPU)	\\
%	MF	&	Mid-frequency	\\
%	MFT	&	Mid-Frequency Telescope	\\
%	MHFT	&	Mid- and High-Frequency Telescopes	\\
%	MKID	&	Microwave kinetic inductance detector	\\
%	MLI	&	Multi-layer insulator	\\
MW & Momentum wheel \\
%	NEP	&	Noise equivalent power	\\
%	NET	&	Noise equivalent temperature	\\
%	NIKA	&	New IRAM KID Array (instrument at IRAM)	\\
%	NIKA2	&	The second generation NIKA experiment	\\
%	NILC	&	Needlet internal linear combination (component-separation algorithm)	\\
%	NIR	&	Near infrared	\\
%	NIST	&	National Institute of Standards and Technology (USA)	\\
%	OBSW	&	On-board software	\\
%	PB 	&	Publication Board	\\
%	PDR	&	Preliminary design review	\\
	PLM	&	Payload module	\\
%	PMC-L	&	PMU controller for LFT	\\
	PMU	&	Polarization modulator unit	\\
%	PO	&	Physical optics	\\
%	POLARBEAR-2	&	A CMB experiment (one of the receivers of the Simons Array)	\\
%	PPR	&	Project preparation review	\\
%	PSM	&	Planck Sky Model	\\
%	PTCD	&	Pulse tube cooler	\\
%	PTCD	&	Pulse tube cooler driver	\\
%	PTEP	&	Progress of Theoretical and Experimental Physics (Journal)	\\
%	QMUL	&	Queen Mary University of London	\\
%	QUAST	&	A module name of GRASP (quasi-optics add-on)	\\
RCS & Reaction Control System \\
%	RCWA	&	Rigorous coupled-wave analysis	\\
%	RF	&	Radio frequency	\\
%	RRR	&	Residual resistance ratio	\\
%	S/C	&	Spacecraft	\\
%	SAA	&	SQUID array amplifier	\\
	SAP	&	Solar array panel	\\
%	SC-A	&	Stirling cooler A	\\
%	SCU	&	SQUID controller unit (suffixes e.g. -L, -M, -H for LFT, MFT, HFT)	\\
%	SCUBA	&	Submillimetre Common-User Bolometer Array 2 (instrument in Hawaii)	\\
%	SGS	&	Science Ground Segment	\\
%	SHI	&	Sumitomo Heavy Industry (company name)	\\
%	SMB	&	Superconducting magnetic bearing	\\
%	SMILES	&	Superconducting Submillimeter-Wave Limb Emission Sounder (on the ISS)	\\
%	SNFR	&	Signal to noise+foregrounds ratio	\\
	SO	&	Simons Observatory (experiment merging ACT & POLARBEAR teams)	\\
%	SPA	&	Signal Processing Assembly (LiteBIRD 300 K FPGA board, a component in each SPU)	\\
%	SPENVIS	&	The Space Environment Information System (www.spenvis.oma.be)	\\
%	SPIDER	&	A balloon-borne CMB experiment	\\
%	SPIRE	&	Spectral and Photometric Imaging Receiver (instrument on Herschel)	\\
	SPO	&	South Pole Observatory (BICEP/Keck + SPT experiments)	\\
%	SPT	&	South Pole Telescope (experiment)	\\
%	SPU	&	Signal Processing Unit (LiteBIRD 300 K FPGA board + digitizers)	\\
%	SQUID	&	Superconducting quantum interference device	\\
%	SS	&	Sun shield	\\
%	SSC	&	Speaker Selection Committee	\\
%	SSL	&	Space Sciences Laboratory (at University of California)	\\
%	STM	&	Structural and thermal model	\\
	STT	&	Star-tracker	\\
	SVM	&	Service module  (synonym: BUS)	\\
%	SWS	&	Sub-wavelength structure	\\
%	SXS	&	X-ray Spectrometer (on Hitomi)	\\
%	TES	&	Transition-edge sensor	\\
%	TIMCO	&		\\
%	TK-RAM	&	The name of the absorber (do we really use this acronym?) - A space-qualified 50-1000GHz absorbing material produced by Thomas Keating Instruments.	\\
%	TMC	&		\\
%	TML	&	Total mass loss	\\
%	TOD	&	Time-ordered data	\\
TOO & Target of opportunity \\
%	TRL	&	Technology readiness level	\\
%	TRP	&	Technology Research Program (in ESA)	\\
%	TSC	&	Tamagawa Seiki Co., Ltd: a motor company in Japan	\\
USC & Uchinoura Space Center \\
%	UMM	&	Universal measurement machine	\\
%	UV	&	Ultraviolet	\\
%	VG	&	V-Groove	\\
%	VNA	&	Vector network analyzer	\\
%	WBS	&	Work Breakdown Structure 	\\
	WMAP	&	Wilkinson Microwave Anisotropy Probe (NASA CMB satellite)	\\
%	YBCO	&	Yttrium barium copper oxide	\\
\hline
\end{tabular}
\caption{}
\end{table}




==> authors_affiliations_LB_2020.01_key_ptep.tex <==
% Ensure the `authblk` package is loaded:
\makeatletter
\@ifpackageloaded{authblk}{}{%
    \@ifpackageloaded{authblk-TI}{}{%
        \usepackage{authblk}% allows handling of the `_authblk.tex` file
    }%
}%
\makeatother

% The following lines handle the prepending/appending of "LiteBIRD Collaboration" for key/general/special papers:
\makeatletter
\def\@author{}
\renewcommand\@author{%
    \ifx\AB@affillist\AB@empty%
        \AB@author%
    \else%
        \ifnum\value{affil}=1%
            \def\rlap##1{##1}\Authfont{\textbf{LiteBIRD Collaboration$\mathbf{^\ast}$\\}}%
        \ifnum\value{affil}>\value{Maxaffil}%
            \def\rlap##1{##1} \AB@authlist \\*[\affilsep] \textbf{$\mathbf{^\ast}$Corresponding E-mail: litebird\_authors@ml.post.kek.jp} \\*[\affilsep]\AB@affillist%
        \fi%
    \fi%
}
\makeatother

% Uncomment the following lines if you want to customize the author and affiliation fonts.
% For font types you can use: normalfont, bfseries, itshape, scshape.
% For font sizes you can use: tiny, scriptsize, footnotesize, small, normalsize, large, Large.
% \renewcommand\Authfont{\normalfont\normalsize}  % normal sized normal font
% \renewcommand\Affilfont{\itshape\small}         % small  sized italic font

\author[1]{E.\,Allys}
\author[2]{K.\,Arnold}
\author[3]{J.\,Aumont}
\author[4]{R.\,Aurlien}
\author[5,6]{S.\,Azzoni}
\author[7,8,9]{C.\,Baccigalupi}
\author[3]{A.\,J.\,Banday}
\author[4]{R.\,Banerji}
\author[10]{R.\,B.\,Barreiro}
\author[11,12,13]{N.\,Bartolo}
\author[3]{L.\,Bautista}
\author[14]{D.\,Beck}
\author[15]{S.\,Beckman}
\author[16,17]{M.\,Bersanelli}
\author[1]{F.\,Boulanger}
\author[4]{M.\,Brilenkov}
\author[18]{M.\,Bucher}
\author[19]{E.\,Calabrese}
\author[20]{P.\,Campeti}
\author[21,22]{A.\,Carones}
\author[10]{F.\,J.\,Casas}
\author[23]{A.\,Catalano}
\author[24]{V.\,Chan}
\author[15,25,26]{K.\,Cheung}
\author[27,6]{Y.\,Chinone}
\author[14,28]{S.\,E.\,Clark}
\author[29,30]{F.\,Columbro}
\author[29,30]{G.\,D'Alessandro}
\author[29,30]{P.\,de\,Bernardis}
\author[31]{T.\,de\,Haan}
\author[10,32]{E.\,de\,la\,Hoz}
\author[29,30]{M.\,De\,Petris}
\author[33]{S.\,Della\,Torre}
\author[10,32]{P.\,Diego-Palazuelos}
\author[34]{M.\,Dobbs}
\author[35,36]{T.\,Dotani}
\author[37]{J.\,M.\,Duval}
\author[38]{T.\,Elleflot}
\author[4]{H.\,K.\,Eriksen}
\author[18]{J.\,Errard}
\author[39]{T.\,Essinger-Hileman}
\author[40,41]{F.\,Finelli}
\author[2]{R.\,Flauger}
\author[16,17]{C.\,Franceschet}
\author[4]{U.\,Fuskeland}
\author[4]{M.\,Galloway}
\author[18]{K.\,Ganga}
\author[42]{M.\,Gerbino}
\author[43,33]{M.\,Gervasi}
\author[44,45]{R.\,T.\,Génova-Santos}
\author[5,6]{T.\,Ghigna}
\author[46]{S.\,Giardiello}
\author[4]{E.\,Gjerløw}
\author[47]{J.\,Grain}
\author[48]{F.\,Grupp}
\author[40,41]{A.\,Gruppuso}
\author[49]{J.\,E.\,Gudmundsson}
\author[50]{N.\,W.\,Halverson}
\author[19]{P.\,Hargrave}
\author[6]{T.\,Hasebe}
\author[51,31,36]{M.\,Hasegawa}
\author[51,31,35,6,36]{M.\,Hazumi}
\author[52]{S.\,Henrot-Versillé}
\author[53]{B.\,Hensley}
\author[54]{L.\,T.\,Hergt}
\author[4]{D.\,Herman}
\author[55]{E.\,Hivon}
\author[24]{R.\,A.\,Hlozek}
\author[15]{A.\,L.\,Hornsby}
\author[56]{Y.\,Hoshino}
\author[57]{J.\,Hubmayr}
\author[58]{K.\,Ichiki}
\author[59]{T.\,Iida}
\author[60]{H.\,Imada}
\author[61]{H.\,Ishino}
\author[50]{G.\,Jaehnig}
\author[6]{N.\,Katayama}
\author[31]{A.\,Kato}
\author[26,15,25]{R.\,Keskitalo}
\author[26]{T.\,Kisner}
\author[62]{Y.\,Kobayashi}
\author[39]{A.\,Kogut}
\author[31]{K.\,Kohri}
\author[20,6]{E.\,Komatsu}
\author[61]{K.\,Komatsu}
\author[63]{K.\,Konishi}
\author[7,8,9]{N.\,Krachmalnicoff}
\author[64,14]{C.\,L.\,Kuo}
\author[29,30]{L.\,Lamagna}
\author[42]{M.\,Lattanzi}
\author[38,15,51]{A.\,T.\,Lee}
\author[18]{C.\,Leloup}
\author[1]{F.\,Levrier}
\author[38,25]{E.\,Linder}
\author[65]{G.\,Luzzi}
\author[23]{J.\,Macias-Perez}
\author[66]{T.\,Maciaszek}
\author[47]{B.\,Maffei}
\author[16]{D.\,Maino}
\author[16,17]{S.\,Mandelli}
\author[10]{E.\,Martínez-González}
\author[29,30]{S.\,Masi}
\author[67]{M.\,Massa}
\author[11,12,13,68]{S.\,Matarrese}
\author[35]{F.\,T.\,Matsuda}
\author[6]{T.\,Matsumura}
\author[29,30]{L.\,Mele}
\author[21,22]{M.\,Migliaccio}
\author[69]{Y.\,Minami}
\author[67]{A.\,Moggi}
\author[34]{J.\,Montgomery}
\author[3]{L.\,Montier}
\author[40]{G.\,Morgante}
\author[3]{B.\,Mot}
\author[61]{Y.\,Nagano}
\author[31]{T.\,Nagasaki}
\author[35]{R.\,Nagata}
\author[70,35]{R.\,Nakano}
\author[6]{T.\,Namikawa}
\author[43,33]{F.\,Nati}
\author[46,42]{P.\,Natoli}
\author[24]{S.\,Nerval}
\author[19]{F.\,Noviello}
\author[35]{K.\,Odagiri}
\author[35]{S.\,Oguri}
\author[62]{H.\,Ohsaki}
\author[46,42,47]{L.\,Pagano}
\author[29,30]{A.\,Paiella}
\author[40,41]{D.\,Paoletti}
\author[43,33]{A.\,Passerini}
\author[18]{G.\,Patanchon}
\author[29,30]{F.\,Piacentini}
\author[18]{M.\,Piat}
\author[65]{G.\,Polenta}
\author[43,33]{D.\,Poletti}
\author[37]{T.\,Prouvé}
\author[21,26]{G.\,Puglisi}
\author[3]{D.\,Rambaud}
\author[15]{C.\,Raum}
\author[16]{S.\,Realini}
\author[20]{M.\,Reinecke}
\author[10,71]{M.\,Remazeilles}
\author[72,47,1]{A.\,Ritacco}
\author[3]{G.\,Roudil}
\author[44,45]{J.\,A.\,Rubino-Martin}
\author[2]{M.\,Russell}
\author[62]{H.\,Sakurai}
\author[61,6]{Y.\,Sakurai}
\author[73]{M.\,Sasaki}
\author[54]{D.\,Scott}
\author[35,70,31]{Y.\,Sekimoto}
\author[74]{K.\,Shinozaki}
\author[75]{M.\,Shiraishi}
\author[39]{P.\,Shirron}
\author[67]{G.\,Signorelli}
\author[67]{F.\,Spinella}
\author[61,6]{S.\,Stever}
\author[18,77]{R.\,Stompor}
\author[56]{S.\,Sugiyama}
\author[54]{R.\,M.\,Sullivan}
\author[26]{A.\,Suzuki}
\author[4]{T.\,L.\,Svalheim}
\author[39]{E.\,Switzer}
\author[78,35]{R.\,Takaku}
\author[70,35]{H.\,Takakura}
\author[61]{Y.\,Takase}
\author[67,79]{A.\,Tartari}
\author[62]{Y.\,Terao}
\author[18]{J.\,Thermeau}
\author[4]{H.\,Thommesen}
\author[64,14]{K.\,L.\,Thompson}
\author[16,17]{M.\,Tomasi}
\author[70,35]{M.\,Tominaga}
\author[52]{M.\,Tristram}
\author[76]{M.\,Tsuji}
\author[35]{M.\,Tsujimoto}
\author[3]{L.\,Vacher}
\author[10]{P.\,Vielva}
\author[21,22]{N.\,Vittorio}
\author[18]{W.\,Wang}
\author[35]{K.\,Watanuki}
\author[4]{I.\,K.\,Wehus}
\author[48]{J.\,Weller}
\author[15]{B.\,Westbrook}
\author[73]{J.\,Wilms}
\author[39]{E.\,J.\,Wollack}
\author[62]{J.\,Yumoto}
\author[43,33]{M.\,Zannoni}
\affil[1]{Laboratoire de Physique de l’École Normale Supérieure, ENS, Université PSL, CNRS, Sorbonne Université, Université de Paris, 75005 Paris, France}
\affil[2]{University of California, San Diego, Department of Physics, San Diego, CA 92093-0424, USA}
\affil[3]{IRAP, Université de Toulouse, CNRS, CNES, UPS, (Toulouse), France}
\affil[4]{Institute of Theoretical Astrophysics, University of Oslo, Blindern, Oslo, Norway}
\affil[5]{Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, United Kingdom}
\affil[6]{Kavli Institute for the Physics and Mathematics of the Universe (Kavli IPMU, WPI), UTIAS, The University of Tokyo, Kashiwa, Chiba 277-8583, Japan}
\affil[7]{International School for Advanced Studies (SISSA), Via Bonomea 265, 34136, Trieste, Italy}
\affil[8]{INFN Sezione di Trieste, via Valerio 2, 34127 Trieste, Italy}
\affil[9]{IFPU, Via Beirut, 2, 34151 Grignano, Trieste, Italy}
\affil[10]{Instituto de Fisica de Cantabria (IFCA, CSIC-UC), Avenida los Castros SN, 39005, Santander, Spain}
\affil[11]{Dipartimento di Fisica e Astronomia “G. Galilei”, Universita` degli Studi di Padova, via Marzolo 8, I-35131 Padova, Italy}
\affil[12]{INFN Sezione di Padova, via Marzolo 8, I-35131, Padova, Italy}
\affil[13]{INAF, Osservatorio Astronomico di Padova, Vicolo dell’Osservatorio 5, I-35122, Padova, Italy}
\affil[14]{Stanford University, Department of Physics,  CA 94305-4060, USA}
\affil[15]{University of California, Berkeley, Department of Physics, Berkeley, CA 94720, USA}
\affil[16]{Dipartimento di Fisica, Universita' degli Studi di Milano, Via Celoria 16 - 20133, Milano, Italy}
\affil[17]{INFN Sezione di Milano, Via Celoria 16 - 20133, Milano, Italy}
\affil[18]{Université de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\affil[19]{School of Physics and Astronomy, Cardiff University, Cardiff CF24 3AA, UK}
\affil[20]{Max Planck Institute for Astrophysics, Karl-Schwarzschild-Str. 1, D-85748 Garching, Germany}
\affil[21]{Dipartimento di Fisica, Università di Roma Tor Vergata, Via della Ricerca Scientifica, 1, 00133, Roma, Italy}
\affil[22]{INFN Sezione di Roma2, Università di Roma Tor Vergata, via della Ricerca Scientifica, 1, 00133 Roma, Italy}
\affil[23]{Univ. Grenoble Alpes, CNRS, LPSC-IN2P3, 53, avenue des Martyrs, 38000 Grenoble, France}
\affil[24]{David A. Dunlap Department of Astronomy and Astrophysics, 50 St. George Street, Toronto ON M5S3H4}
\affil[25]{University of California, Berkeley, Space Sciences Laboratory,  Berkeley, CA 94720, USA}
\affil[26]{Lawrence Berkeley National Laboratory (LBNL), Computational Cosmology Center, Berkeley, CA 94720, USA}
\affil[27]{University of Tokyo, School of Science, Research Center for the Early Universe, RESCEU}
\affil[28]{Kavli Institute for Particle Astrophysics and Cosmology (KIPAC), Stanford University, Stanford, CA 94305, USA}
\affil[29]{Dipartimento di Fisica, Università La Sapienza, P. le A. Moro 2, Roma, Italy}
\affil[30]{INFN Sezione di Roma, P.le A. Moro 2, 00185 Roma, Italy}
\affil[31]{Institute of Particle and Nuclear Studies (IPNS), High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan}
\affil[32]{Dpto. de Física Moderna, Universidad de Cantabria, Avda. los Castros s/n, E-39005 Santander, Spain}
\affil[33]{INFN Sezione Milano Bicocca, Piazza della Scienza, 3, 20126 Milano, Italy}
\affil[34]{McGill University, Physics Department, Montreal, QC H3A 0G4, Canada}
\affil[35]{Japan Aerospace Exploration Agency (JAXA), Institute of Space and Astronautical Science (ISAS), Sagamihara, Kanagawa 252-5210, Japan}
\affil[36]{The Graduate University for Advanced Studies (SOKENDAI), Miura District, Kanagawa 240-0115, Hayama, Japan}
\affil[37]{Université Grenoble Alpes, CEA, IRIG-DSBT, 38000 Grenoble, France}
\affil[38]{Lawrence Berkeley National Laboratory (LBNL), Physics Division, Berkeley, CA 94720, USA}
\affil[39]{NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\affil[40]{INAF - OAS Bologna, via Piero Gobetti, 93/3, 40129 Bologna (Italy)}
\affil[41]{INFN Sezione di Bologna, Viale C. Berti Pichat, 6/2 – 40127 Bologna Italy}
\affil[42]{INFN Sezione di Ferrara, Via Saragat 1, 44122 Ferrara, Italy}
\affil[43]{University of Milano Bicocca, Physics Department, p.zza della Scienza, 3, 20126 Milan Italy}
\affil[44]{Instituto de Astrofísica de Canarias, E-38200 La Laguna, Tenerife, Canary Islands, Spain}
\affil[45]{Departamento de Astrofísica, Universidad de La Laguna (ULL), E-38206, La Laguna, Tenerife, Spain}
\affil[46]{Dipartimento di Fisica e Scienze della Terra, Università di Ferrara, Via Saragat 1, 44122 Ferrara, Italy}
\affil[47]{Université Paris-Saclay, CNRS, Institut d’Astrophysique Spatiale, 91405, Orsay, France.}
\affil[48]{Universitäts-Sternwarte, Fakultät für Physik, Ludwig-Maximilians Universität München, Scheinerstr.1, 81679 München, Germany}
\affil[49]{The Oskar Klein Centre, Department of Physics, Stockholm University, SE-106 91 Stockholm, Sweden}
\affil[50]{Center for Astrophysics and Space Astronomy, University of Colorado, Boulder, CO, 80309, USA}
\affil[51]{International Center for Quantum-field Measurement Systems for Studies of the Universe and Particles (QUP), High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan}
\affil[52]{Université Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affil[53]{Department of Astrophysical Sciences, Peyton Hall, Princeton University, Princeton, NJ, USA 08544}
\affil[54]{Department of Physics and Astronomy, University of British Columbia, 6224 Agricultural Road, Vancouver BC, V6T1Z1, Canada}
\affil[55]{Institut d'Astrophysique de Paris, CNRS/Sorbonne Université, Paris France}
\affil[56]{Saitama University, Saitama 338-8570, Japan}
\affil[57]{NIST Quantum Sensors Group, 325 Broadway, Boulder, CO 80305, USA}
\affil[58]{Nagoya University, Kobayashi-Masukawa Institute for the Origin of Particle and the Universe, Aichi 464-8602, Japan}
\affil[59]{ispace, inc.}
\affil[60]{National Astronomical Observatory of Japan, Mitaka, Tokyo 181-8588, Japan}
\affil[61]{Okayama University, Department of Physics, Okayama 700-8530, Japan}
\affil[62]{The Institute for Solid State Physics (ISSP), The University of Tokyo, Kashiwa, Chiba 277-8581, Japan}
\affil[63]{The University of Tokyo, Institute for Photon Science and Technology}
\affil[64]{SLAC National Accelerator Laboratory, Kavli Institute for Particle Astrophysics and Cosmology (KIPAC),  Menlo Park, CA 94025, USA}
\affil[65]{Space Science Data Center, Italian Space Agency, via del Politecnico, 00133, Roma, Italy}
\affil[66]{Centre National d'Etudes Spatiales (CNES), France}
\affil[67]{INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa (Italy)}
\affil[68]{Gran Sasso Science Institute (GSSI), Viale F. Crispi 7, I-67100, L’Aquila, Italy}
\affil[69]{Research Center for Nuclear Physics, Osaka University, Ibaraki, Osaka, 567-0047, Japan}
\affil[70]{The University of Tokyo, Department of Astronomy, Tokyo 113-0033, Japan}
\affil[71]{Jodrell Bank Centre for Astrophysics, Department of Physics and Astronomy, School of Natural Sciences, The University of Manchester, Oxford Road, Manchester M13 9PL, UK}
\affil[72]{INAF-Osservatorio Astronomico di Cagliari, Via della Scienza 5, 09047 Selargius, IT}
\affil[73]{Remeis-Observatory and Erlangen Centre for Astroparticle Physics, FAU Erlangen-Nürnberg, Sternwartstr. 7, 96049 Bamberg, Germany}
\affil[74]{Japan Aerospace Exploration Agency (JAXA), Research and Development Directorate, Tsukuba, Ibaraki 305-8505, Japan}
\affil[75]{School of General and Management Studies, Suwa University of Science, 5000-1 Toyohira, Chino, Nagano 391-0292, Japan}
\affil[76]{National Institute of Technology, Kagawa College}
\affil[77]{CNRS-UCB International Research Laboratory, Centre Pierre Binétruy, UMI2007, Berkeley, CA94720, USA}
\affil[78]{The University of Tokyo, Department of Physics, Tokyo 113-0033, Japan}
\affil[79]{Dipartimento di Fisica, Università di Pisa, Largo B. Pontecorvo 3, 56127 Pisa}


==> authors_affiliations_LB_2020.01_key_ptepv2.tex <==
% Ensure the `authblk` package is loaded:
\makeatletter
\@ifpackageloaded{authblk}{}{%
    \@ifpackageloaded{authblk-TI}{}{%
        \usepackage{authblk}% allows handling of the `_authblk.tex` file
    }%
}%
\makeatother

% The following lines handle the prepending/appending of "LiteBIRD Collaboration" for key/general/special papers:
\makeatletter
\def\@author{}
\renewcommand\@author{%
    \ifx\AB@affillist\AB@empty%
        \AB@author%
    \else%
        \ifnum\value{affil}=1%
            \def\rlap##1{##1}\Authfont{\textbf{LiteBIRD Collaboration$\mathbf{^\ast}$\\}}%
        \ifnum\value{affil}>\value{Maxaffil}%
            \def\rlap##1{##1} \AB@authlist \\*[\affilsep] \textbf{$\mathbf{^\ast}$Corresponding E-mail: litebird\_authors@ml.post.kek.jp} \\*[\affilsep]\AB@affillist%
        \fi%
    \fi%
}
\makeatother

% Uncomment the following lines if you want to customize the author and affiliation fonts.
% For font types you can use: normalfont, bfseries, itshape, scshape.
% For font sizes you can use: tiny, scriptsize, footnotesize, small, normalsize, large, Large.
% \renewcommand\Authfont{\normalfont\normalsize}  % normal sized normal font
% \renewcommand\Affilfont{\itshape\small}         % small  sized italic font

\author[1]{E.\,Allys}
\author[2]{K.\,Arnold}
\author[3]{J.\,Aumont}
\author[4]{R.\,Aurlien}
\author[5,6]{S.\,Azzoni}
\author[7,8,9]{C.\,Baccigalupi}
\author[3]{A.\,J.\,Banday}
\author[4]{R.\,Banerji}
\author[10]{R.\,B.\,Barreiro}
\author[11,12,13]{N.\,Bartolo}
\author[3]{L.\,Bautista}
\author[14]{D.\,Beck}
\author[15]{S.\,Beckman}
\author[16,17]{M.\,Bersanelli}
\author[1]{F.\,Boulanger}
\author[4]{M.\,Brilenkov}
\author[18]{M.\,Bucher}
\author[19]{E.\,Calabrese}
\author[20]{P.\,Campeti}
\author[21,22]{A.\,Carones}
\author[10]{F.\,J.\,Casas}
\author[23]{A.\,Catalano}
\author[24]{V.\,Chan}
\author[15,25,26]{K.\,Cheung}
\author[6,27]{Y.\,Chinone}
\author[14,28]{S.\,E.\,Clark}
\author[29,30]{F.\,Columbro}
\author[29,30]{G.\,D'Alessandro}
\author[29,30]{P.\,de\,Bernardis}
\author[31]{T.\,de\,Haan}
\author[10,32]{E.\,de\,la\,Hoz}
\author[29,30]{M.\,De\,Petris}
\author[33]{S.\,Della\,Torre}
\author[10,32]{P.\,Diego-Palazuelos}
\author[34]{M.\,Dobbs}
\author[35,36]{T.\,Dotani}
\author[37]{J.\,M.\,Duval}
\author[38]{T.\,Elleflot}
\author[4]{H.\,K.\,Eriksen}
\author[18]{J.\,Errard}
\author[39]{T.\,Essinger-Hileman}
\author[40,41]{F.\,Finelli}
\author[2]{R.\,Flauger}
\author[16,17]{C.\,Franceschet}
\author[4]{U.\,Fuskeland}
\author[4]{M.\,Galloway}
\author[18]{K.\,Ganga}
\author[42]{M.\,Gerbino}
\author[33,43]{M.\,Gervasi}
\author[44,45]{R.\,T.\,Génova-Santos}
\author[5,6]{T.\,Ghigna}
\author[46]{S.\,Giardiello}
\author[4]{E.\,Gjerløw}
\author[47]{J.\,Grain}
\author[48]{F.\,Grupp}
\author[40,41]{A.\,Gruppuso}
\author[49]{J.\,E.\,Gudmundsson}
\author[50]{N.\,W.\,Halverson}
\author[19]{P.\,Hargrave}
\author[6]{T.\,Hasebe}
\author[31,36,51]{M.\,Hasegawa}
\author[6,31,35,36,51]{M.\,Hazumi}
\author[52]{S.\,Henrot-Versillé}
\author[53]{B.\,Hensley}
\author[54]{L.\,T.\,Hergt}
\author[4]{D.\,Herman}
\author[55]{E.\,Hivon}
\author[24]{R.\,A.\,Hlozek}
\author[15]{A.\,L.\,Hornsby}
\author[56]{Y.\,Hoshino}
\author[57]{J.\,Hubmayr}
\author[58]{K.\,Ichiki}
\author[59]{T.\,Iida}
\author[60]{H.\,Imada}
\author[61]{H.\,Ishino}
\author[50]{G.\,Jaehnig}
\author[6]{N.\,Katayama}
\author[31]{A.\,Kato}
\author[15,25,26]{R.\,Keskitalo}
\author[26]{T.\,Kisner}
\author[62]{Y.\,Kobayashi}
\author[39]{A.\,Kogut}
\author[31]{K.\,Kohri}
\author[6,20]{E.\,Komatsu}
\author[61]{K.\,Komatsu}
\author[63]{K.\,Konishi}
\author[7,8,9]{N.\,Krachmalnicoff}
\author[14,64]{C.\,L.\,Kuo}
\author[29,30]{L.\,Lamagna}
\author[42]{M.\,Lattanzi}
\author[15,38,51]{A.\,T.\,Lee}
\author[18]{C.\,Leloup}
\author[1]{F.\,Levrier}
\author[25,38]{E.\,Linder}
\author[65]{G.\,Luzzi}
\author[23]{J.\,Macias-Perez}
\author[66]{T.\,Maciaszek}
\author[47]{B.\,Maffei}
\author[16]{D.\,Maino}
\author[16,17]{S.\,Mandelli}
\author[10]{E.\,Martínez-González}
\author[29,30]{S.\,Masi}
\author[67]{M.\,Massa}
\author[11,12,13,68]{S.\,Matarrese}
\author[35]{F.\,T.\,Matsuda}
\author[6]{T.\,Matsumura}
\author[29,30]{L.\,Mele}
\author[21,22]{M.\,Migliaccio}
\author[69]{Y.\,Minami}
\author[67]{A.\,Moggi}
\author[34]{J.\,Montgomery}
\author[3]{L.\,Montier}
\author[40]{G.\,Morgante}
\author[3]{B.\,Mot}
\author[61]{Y.\,Nagano}
\author[31]{T.\,Nagasaki}
\author[35]{R.\,Nagata}
\author[35,70]{R.\,Nakano}
\author[6]{T.\,Namikawa}
\author[33,43]{F.\,Nati}
\author[42,46]{P.\,Natoli}
\author[24]{S.\,Nerval}
\author[19]{F.\,Noviello}
\author[35]{K.\,Odagiri}
\author[35]{S.\,Oguri}
\author[62]{H.\,Ohsaki}
\author[42,46,47]{L.\,Pagano}
\author[29,30]{A.\,Paiella}
\author[40,41]{D.\,Paoletti}
\author[33,43]{A.\,Passerini}
\author[18]{G.\,Patanchon}
\author[29,30]{F.\,Piacentini}
\author[18]{M.\,Piat}
\author[19,29,30]{G.\,Pisano}  %newly added
\author[65]{G.\,Polenta}
\author[33,43]{D.\,Poletti}
\author[37]{T.\,Prouvé}
\author[21,26]{G.\,Puglisi}
\author[3]{D.\,Rambaud}
\author[15]{C.\,Raum}
\author[16]{S.\,Realini}
\author[20]{M.\,Reinecke}
\author[10,71]{M.\,Remazeilles}
\author[1,47,72]{A.\,Ritacco}
\author[3]{G.\,Roudil}
\author[44,45]{J.\,A.\,Rubino-Martin}
\author[2]{M.\,Russell}
\author[62]{H.\,Sakurai}
\author[6,61]{Y.\,Sakurai}
\author[73]{M.\,Sasaki}
\author[54]{D.\,Scott}
\author[31,35,70]{Y.\,Sekimoto}
\author[74]{K.\,Shinozaki}
\author[75]{M.\,Shiraishi}
\author[39]{P.\,Shirron}
\author[67]{G.\,Signorelli}
\author[67]{F.\,Spinella}
\author[6,61]{S.\,Stever}
\author[18,76]{R.\,Stompor}  
\author[56]{S.\,Sugiyama}
\author[54]{R.\,M.\,Sullivan}
\author[26]{A.\,Suzuki}
\author[4]{T.\,L.\,Svalheim}
\author[39]{E.\,Switzer}
\author[35,77]{R.\,Takaku}
\author[35,70]{H.\,Takakura}
\author[61]{Y.\,Takase}
\author[67,78]{A.\,Tartari} 
\author[62]{Y.\,Terao}
\author[18]{J.\,Thermeau}
\author[4]{H.\,Thommesen}
\author[14,64]{K.\,L.\,Thompson}
\author[16,17]{M.\,Tomasi}
\author[35,70]{M.\,Tominaga}
\author[52]{M.\,Tristram}
\author[79]{M.\,Tsuji} 
\author[35]{M.\,Tsujimoto}
\author[3]{L.\,Vacher}
\author[10]{P.\,Vielva}
\author[21,22]{N.\,Vittorio}
\author[18]{W.\,Wang}
\author[35]{K.\,Watanuki}
\author[4]{I.\,K.\,Wehus}
\author[48]{J.\,Weller}
\author[15]{B.\,Westbrook}
\author[73]{J.\,Wilms}
\author[80,81]{B.\,Winter}  %newly added
\author[39]{E.\,J.\,Wollack}
\author[62]{J.\,Yumoto}
\author[33,43]{M.\,Zannoni}
\affil[1]{Laboratoire de Physique de l’École Normale Supérieure, ENS, Université PSL, CNRS, Sorbonne Université, Université de Paris, F-75005 Paris, France}
\affil[2]{University of California, San Diego, Department of Physics, San Diego, CA 92093-0424, USA}
\affil[3]{IRAP, Université de Toulouse, CNRS, CNES, UPS (Toulouse), 9 avenue du Colonel Roche BP 44346, F-31028 Toulouse Cedex 4, France}
\affil[4]{Institute of Theoretical Astrophysics, University of Oslo, Blindern 0315, Oslo, Norway}
\affil[5]{Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK}
\affil[6]{Kavli Institute for the Physics and Mathematics of the Universe (Kavli IPMU, WPI), UTIAS, The University of Tokyo, Kashiwa, Chiba 277-8583, Japan}
\affil[7]{International School for Advanced Studies (SISSA), Via Bonomea 265, I-34136 Trieste, Italy}
\affil[8]{INFN Sezione di Trieste, Via Valerio 2, I-34127 Trieste, Italy}
\affil[9]{IFPU, Via Beirut, 2, I-34151 Grignano, Trieste, Italy}
\affil[10]{Instituto de Fisica de Cantabria (IFCA, CSIC-UC), Avenida los Castros SN, E-39005 Santander, Spain}
\affil[11]{Dipartimento di Fisica e Astronomia “G. Galilei”, Universita` degli Studi di Padova, Via Marzolo 8, I-35131 Padova, Italy}
\affil[12]{INFN Sezione di Padova, via Marzolo 8, I-35131 Padova, Italy}
\affil[13]{INAF, Osservatorio Astronomico di Padova, Vicolo dell’Osservatorio 5, I-35122 Padova, Italy}
\affil[14]{Stanford University, Department of Physics, CA 94305-4060, USA}
\affil[15]{University of California, Berkeley, Department of Physics, Berkeley, CA 94720, USA}
\affil[16]{Dipartimento di Fisica, Universita' degli Studi di Milano, Via Celoria 16, I-20133 Milano, Italy}
\affil[17]{INFN Sezione di Milano, Via Celoria 16, I-20133 Milano, Italy}
\affil[18]{Université de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\affil[19]{School of Physics and Astronomy, Cardiff University, Cardiff CF24 3AA, UK}
\affil[20]{Max Planck Institute for Astrophysics, Karl-Schwarzschild-Str. 1, D-85748 Garching, Germany}
\affil[21]{Dipartimento di Fisica, Università di Roma Tor Vergata, Via della Ricerca Scientifica 1, I-00133 Roma, Italy}
\affil[22]{INFN Sezione di Roma2, Università di Roma Tor Vergata, Via della Ricerca Scientifica 1, I-00133 Roma, Italy}
\affil[23]{Univ. Grenoble Alpes, CNRS, LPSC-IN2P3, 53 avenue des Martyrs, F-38000 Grenoble, France}
\affil[24]{David A. Dunlap Department of Astronomy and Astrophysics, 50 St George Street, Toronto ON M5S 3H4, Canada}
\affil[25]{University of California, Berkeley, Space Sciences Laboratory,  Berkeley, CA 94720, USA}
\affil[26]{Lawrence Berkeley National Laboratory (LBNL), Computational Cosmology Center, Berkeley, CA 94720, USA}
\affil[27]{University of Tokyo, School of Science, Research Center for the Early Universe, RESCEU, Tokyo 113-0033, Japan}
\affil[28]{Kavli Institute for Particle Astrophysics and Cosmology (KIPAC), Stanford University, Stanford, CA 94305, USA}
\affil[29]{Dipartimento di Fisica, Università La Sapienza, P.le A. Moro 2, I-00185 Roma, Italy}
\affil[30]{INFN Sezione di Roma, P.le A. Moro 2, I-00185 Roma, Italy}
\affil[31]{Institute of Particle and Nuclear Studies (IPNS), High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan}
\affil[32]{Dpto. de Física Moderna, Universidad de Cantabria, Avda. los Castros s/n, E-39005 Santander, Spain}
\affil[33]{INFN Sezione Milano Bicocca, Piazza della Scienza, 3, I-20126 Milano, Italy}
\affil[34]{McGill University, Physics Department, Montreal, QC H3A 0G4, Canada}
\affil[35]{Japan Aerospace Exploration Agency (JAXA), Institute of Space and Astronautical Science (ISAS), Sagamihara, Kanagawa 252-5210, Japan}
\affil[36]{The Graduate University for Advanced Studies (SOKENDAI), Miura District, Kanagawa 240-0115, Hayama, Japan}
\affil[37]{Université Grenoble Alpes, CEA, IRIG-DSBT, F-38000 Grenoble, France}
\affil[38]{Lawrence Berkeley National Laboratory (LBNL), Physics Division, Berkeley, CA 94720, USA}
\affil[39]{NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\affil[40]{INAF - OAS Bologna, Via Piero Gobetti, 93/3, I-40129 Bologna, Italy}
\affil[41]{INFN Sezione di Bologna, Viale C. Berti Pichat, 6/2 I-40127 Bologna, Italy}
\affil[42]{INFN Sezione di Ferrara, Via Saragat 1, I-44122 Ferrara, Italy}
\affil[43]{University of Milano Bicocca, Physics Department, p.zza della Scienza, 3, I-20126 Milan, Italy}
\affil[44]{Instituto de Astrofísica de Canarias, E-38200 La Laguna, Tenerife, Canary Islands, Spain}
\affil[45]{Departamento de Astrofísica, Universidad de La Laguna (ULL), E-38206 La Laguna, Tenerife, Spain}
\affil[46]{Dipartimento di Fisica e Scienze della Terra, Università di Ferrara, Via Saragat 1, I-44122 Ferrara, Italy}
\affil[47]{Université Paris-Saclay, CNRS, Institut d’Astrophysique Spatiale, F-91405 Orsay, France.}
\affil[48]{Universitäts-Sternwarte, Fakultät für Physik, Ludwig-Maximilians Universität München, Scheinerstr.1, D-81679 München, Germany}
\affil[49]{The Oskar Klein Centre, Department of Physics, Stockholm University, SE-106 91 Stockholm, Sweden}
\affil[50]{Center for Astrophysics and Space Astronomy, University of Colorado, Boulder, CO 80309, USA}
\affil[51]{International Center for Quantum-field Measurement Systems for Studies of the Universe and Particles (QUP), High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan}
\affil[52]{Université Paris-Saclay, CNRS/IN2P3, IJCLab, F-91405 Orsay, France}
\affil[53]{Department of Astrophysical Sciences, Peyton Hall, Princeton University, Princeton, NJ 08544, USA}
\affil[54]{Department of Physics and Astronomy, University of British Columbia, 6224 Agricultural Road, Vancouver, BC V6T 1Z1, Canada}
\affil[55]{Institut d'Astrophysique de Paris, CNRS/Sorbonne Université, Paris, France}
\affil[56]{Saitama University, Saitama 338-8570, Japan}
\affil[57]{NIST Quantum Sensors Group, 325 Broadway, Boulder, CO 80305, USA}
\affil[58]{Nagoya University, Kobayashi-Masukawa Institute for the Origin of Particle and the Universe, Aichi 464-8602, Japan}
\affil[59]{ispace, inc., Tokyo 103-0007, Japan}
\affil[60]{National Astronomical Observatory of Japan, Mitaka, Tokyo 181-8588, Japan}
\affil[61]{Okayama University, Department of Physics, Okayama 700-8530, Japan}
\affil[62]{The Institute for Solid State Physics (ISSP), The University of Tokyo, Kashiwa, Chiba 277-8581, Japan}
\affil[63]{The University of Tokyo, Institute for Photon Science and Technology, 113-0033, Japan}
\affil[64]{SLAC National Accelerator Laboratory, Kavli Institute for Particle Astrophysics and Cosmology (KIPAC),  Menlo Park, CA 94025, USA}
\affil[65]{Space Science Data Center, Italian Space Agency, Via del Politecnico, I-00133, Roma, Italy}
\affil[66]{Centre National d'Etudes Spatiales (CNES), 18 avenue Edouard Belin  31 401 TOULOUSE CEDEX 4, France}
\affil[67]{INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, I-56127 Pisa, Italy}
\affil[68]{Gran Sasso Science Institute (GSSI), Viale F. Crispi 7, I-67100, L’Aquila, Italy}
\affil[69]{Research Center for Nuclear Physics, Osaka University, Ibaraki, Osaka, 567-0047, Japan}
\affil[70]{The University of Tokyo, Department of Astronomy, Tokyo 113-0033, Japan}
\affil[71]{Jodrell Bank Centre for Astrophysics, Department of Physics and Astronomy, School of Natural Sciences, The University of Manchester, Oxford Road, Manchester M13 9PL, UK}
\affil[72]{INAF-Osservatorio Astronomico di Cagliari, Via della Scienza 5, I-09047 Selargius, Italy}
\affil[73]{Remeis-Observatory and Erlangen Centre for Astroparticle Physics, FAU Erlangen-Nürnberg, Sternwartstr. 7, D-96049 Bamberg, Germany}
\affil[74]{Japan Aerospace Exploration Agency (JAXA), Research and Development Directorate, Tsukuba, Ibaraki 305-8505, Japan}
\affil[75]{School of General and Management Studies, Suwa University of Science, 5000-1 Toyohira, Chino, Nagano 391-0292, Japan}
\affil[76]{CNRS-UCB International Research Laboratory, Centre Pierre Binétruy, UMI2007, Berkeley, CA94720, USA}
\affil[77]{The University of Tokyo, Department of Physics, Tokyo 113-0033, Japan}
\affil[78]{Dipartimento di Fisica, Università di Pisa, Largo B. Pontecorvo 3, I-56127 Pisa, Italy}
\affil[79]{National Institute of Technology, Kagawa College, Kagawa 761-8058, Japan}
\affil[80]{Physics and Astronomy Dept., University College London (UCL), London}
\affil[81]{Mullard Space Science Laboratory, University College London, Surrey RH5 6NT, UK}

